Knowledge-Aware Language Model Pretraining

How much knowledge do pretrained language models hold? Recent research observed that pretrained transformers are adept at modeling semantics but it is unclear to what degree they grasp human knowledge, or how to ensure they do so. In this paper we incorporate knowledge-awareness in language model pretraining without changing the transformer architecture, inserting explicit knowledge layers, or adding external storage of semantic information. Rather, we simply signal the existence of entities to the input of the transformer in pretraining, with an entity-extended tokenizer; and at the output, with an additional entity prediction task. Our experiments show that solely by adding these entity signals in pretraining, significantly more knowledge is packed into the transformer parameters: we observe improved language modeling accuracy, factual correctness in LAMA knowledge probing tasks, and semantics in the hidden representations through edge probing.We also show that our knowledge-aware language model (KALM) can serve as a drop-in replacement for GPT-2 models, significantly improving downstream tasks like zero-shot question-answering with no task-related training.

==> arxiv/application.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{l|ll|ll|ll}
    \multicolumn{1}{c|}{Model} & \multicolumn{2}{c|}{Trivia QA}                      & \multicolumn{2}{c|}{Natural Questions}              & \multicolumn{2}{c|}{Web Questions}                 \\
    @100k chkpt                & \multicolumn{1}{c}{EM} & \multicolumn{1}{c|}{in-EM} & \multicolumn{1}{c}{EM} & \multicolumn{1}{c|}{in-EM} & \multicolumn{1}{c}{EM} & \multicolumn{1}{c}{in-EM} \\ \hline
    T5-B                       & 29.1                   & -                          & 27.0                   & -                          & 29.1                   & -                         \\
    T5-L                       & 35.9                   & -                          & 29.8                   & -                          & 32.2                   & -                         \\
    T5-11B                     & 50.1                   & -                          & 34.5                   & -                          & 37.4                   & -                         \\ \hline
    TNLG-12L                   & 0.0344                 & 0.0477                     & 0.0081                 & 0.0124                     & 0.0208                 & 0.0292                    \\
    TNLG-24L                   & 0.0625+                & 0.0778                     & 0.0273                 & 0.0346                     & 0.0349                 & 0.0542                    \\
    TNLG-1.5B                  & 0.1778+                & 0.2159+                    & 0.0608+                & 0.0795+                    & 0.0620+                & 0.1265+                   \\
    TNLG-17B                   & 0.4232                 & 0.4756                     & 0.1434                 & 0.1730                     & 0.1215                 & 0.2168                    \\ \hline
    KALM-12L                   & 0.0587                 & 0.0716                     & 0.0175                 & 0.0213                     & 0.0353                 & 0.0479                    \\
    KALM-24L                   & 0.0867                 & 0.0999                     &                        &                            &                        &                          
    \end{tabular}
    \caption{Zero-shot question answering performance of different models at the 100k checkpoint of training for three different question answering benchmarks. EM is exact match percent, and in-EM is the percent correct when counting whether the correct answer is a substring of the generated answer. All generated answers were generated by a greedy decoding of at most 20 tokens. \cx{T5 is not zero-shot and we don't need to compare with it? Show the best one T5-11B and say it is fully-supervised and as an upper bound is fine.}}
    \label{tab:application}
\end{table}

==> arxiv/eva.tex <==
\section{Evaluation Results}

\subsection{Language Modeling and Knowledge Probing Results}
In Table ~\ref{tab:lmoverall} we show both the language modeling tasks Wikitext (perplexity) and Lambada (last word accuracy), adjacent to the LAMA average precision at 1 results on its four relation categories. In general, the \tnlg{} results are slightly better than the Open AI models of equivalent architecture due to more training data. More importantly, we consistently see that \kalm{} has around 10-15\% improvement on perplexity and LAMBADA accuracy, but on LAMA knowledge probe which directly tests whether the model can complete factual statements, \kalm{} consistently improves over \tnlg{} by margins of 40-80\%, even approaching performance of a \tnlg{} model with twice as many transformer parameters. \kalm{} clearly generates more factually correct text simply by being aware of the existence of entities in its context. 

The improvement is most noticeable on T-Rex, which tests hundreds of knowledge base relations like ``X is owned by Y'' where the object X is given but the model must complete Y. Similarly for Squad, over 300 questions were rewritten such that their answer could be filled in at the end of the sentence like T-Rex. Concept-Net however does not test for relationships between entities and is therefore less impacted by our method. 

\input{table/overall}

% \cx{Things to discuss:
% \begin{enumerate}
%     \item Describe the overall table
%     \item discuss our advantage on the LM and lamada test at the same parameter level or competing with bigger GPT-2 versions
%     \item discuss our advantage on LAMA, the different advantage on different tasks and why
%     \item discuss the overall conclusion from this experiment, that \kalm{} does have better knowledge capability simply with knowledge aware pretraining
% \end{enumerate}
% }


\subsection{Zero-Shot Task Performances}
In Table ~\ref{tab:application} we compare the zero-shot question answering performance of \tnlg{} and \kalm{} models, as well as T5 which was trained in a supervised fashion on the train splits of these QA datasets. Remarkably, even though the largest \tnlg{} model was only trained on unsupervised text prediction tasks, it still performs nearly as well as the fully-supervised T5 11B model, showing that indeed, larger language models do capture knowledge without supervision. 

However, our \kalm{} models more efficiently pack both language and factual information into their parameters without sacrificing speed: the 12L \kalm{} Base is very close to the zero shot accuracy of the 24L \tnlg{} Large. Furthermore, the extra entity embeddings in \kalm{} models do not significantly increase runtime -- they are constant time lookup operations after a linear time entity linking operation. This is crucial, as many other knowledge-grounded models use special ``knowledge transformer'' layers in addition to the normal transformer layers which will increase runtime.  

\input{table/application}

Natural Questions and Web Questions are more similar to what real world users ask to a search engine, so they are naturally more related to recent and local events or information. Trivia QA, on the other hand, contains more cut-and-dry questions typically about historical events. 

% \cx{Use figures instead of tables in this evaluation results, check the plot in GPT-2 paper in zero-shot QA}

% \cx{Things to discuss:
% \begin{enumerate}
%     \item describe the figures. make sure stating that this is zero-shot, the T5 STOA numbers are fully supervised and is different. (adding KA to these nonautogressive LMs is a future work)
%     \item describe the zero-shot acc w.r.t. model capacity, reconfirm GPT-2's and scaling law's observation.
%     \item describe our gains on different tasks over GPT-2
%     \item conclude that the improved knowledge learning capability also leads to better zero-shot task performances
% \end{enumerate}
% }




\subsection{Captured Semantics During Knowledge Aware Pretraining}
In addition to comparing the performance of converged models, we also analyze the learning progress of the models \textit{at different steps of training} before convergence. Shown in Figure~\ref{fig:performance_probe_tasks}, KALM Base starts demonstrating its higher quality over GPT Base given adequate pretraining (5k-10k steps); while the earlier lags could be explained by the training used to learn meaningful entity embeddings. Furthermore, KALM Base performs better on entity-oriented tasks like named entity typing (Entities), which is attributed to its adoption of the entity embedding layer.

Semantic-oriented tasks such as relation classification (Relations) require a higher level of linguistic understanding to capture the local semantics as well as the long range dependency. In these tasks, both PLMs needs more prior training to reach a satisfactory convergence level. In contrast, on syntax-oriented tasks such as dependency labeling (Deps) or POS tagging (POS), these PLMs achieve a competitive performance even at earlier training steps. This result hints that shallower linguistic knowledge is captured first in the language model pretraining.

\begin{figure}
    \centering
    \includegraphics[trim=10 0 10 0, clip, scale=0.62]{performance_probe_tasks.eps}
    \caption{The fine-tuning result of the 12-layer \tnlg~ Base and \kalm~ Base models on 8 Edge Probe tasks. We evaluate both encoders at different pretraining checkpoints. Values on x-axis are the numbers of pretraining steps. Scores on y-axis are the micro-averaged $F_1$ performance.}
    \label{fig:performance_probe_tasks}
\end{figure}

\cx{Use the eight subfigures in a row, each one with \tnlg{} and \kalm{} F1 (y) at different training steps (x). tweak the scale of x-axis to better illustrate the tread}
\cx{Things to discuss
\begin{enumerate}
    \item describe the figure
    \item compare different tasks and deliver the intuition which ones are easier and which ones are more higher order and long range semantics
    \item describe the performance on different level's semantic tasks (low 4 vs high 4) along the training steps. which information is captured earlier, and which is captured later
    \item compare \kalm{} and \tnlg{} and show what is better captured at the final F1
    \item compare the two and discuss the differences in the pretraining steps: e.g., kalm may capture something much sooner.
\end{enumerate}
}

\input{table/learninganalyses}






==> arxiv/exp.tex <==
\input{table/exp}
\section{Experimental Methodologies}
In this section we describe our general experimental settings. All open-source tools and datasets are used following their standard settings unless described. More details can be found in Appendix.

\textbf{Pretraining with Knowledge Awareness.} 
We use a pretraining dataset similar to OpenWebText\footnote{https://github.com/NVIDIA/Megatron-LM/tree/master/tools/openwebtext} with an expanded list of URLs; it contains about 30 billion tokens after filtering and deduplication. We keep this dataset fixed for all \tnlg{{} and \kalm{} experiments in this paper.  

The entity toknizer in \kalm{} uses the entity dictionary from the CMNS Linker~\cite{hasibi2017entity}, which was harvested from the FACC1 and FAKBA entity annotations~\cite{gabrilovich2013facc1}.  We keep surface forms with frequency at least 1k and entities with at least 100, in total about 1.4M entities. The tokenizer uses forward-greedy and maps the longest (at most 4-grams) surface form to their most popular entity~\cite{hasibi2017entity}. 

We choose this frequency based dictionary lookup to favor coverage, efficiency, and similarity, while rely on the language model pretraining to handle the linking noises~\cite{xiong2017duet}.


\textbf{Evaluations.} We first evaluate all pretrained language models using perplexity on WikiText-103~\cite{merity2016pointer} by perplexity and accuracy in LAMBADA last-word prediction task~\cite{hoang-etal-2018-entity}, using their standard settings and following Megatron-LM's implementation~\cite{shoeybi2019megatron}.  

% We evaluate all our trained models on the generic generative language model benchmarks of wikiText-103~\cite{merity2016pointer} test perplexity and LAMBADA  last-word prediction~\cite{hoang-etal-2018-entity}, following the same format as the Megatron-LM codebase~\cite{shoeybi2019megatron}. Importantly, LAMBADA is evaluated such that the entire last word must be predicted (if it is more than one token, all must be predicted correctly) without telling the model in any way that it is indeed the last word of a sentence. 

A description of all the evaluation datasets can be found in Table ~\ref{tab:datasizes}. 



We also use the LAMA knowledge probe~\cite{petroni2019lama} to report the sample average precision at 1 answers generated by the model on each of the four categories of relations: Squad, Concept Net, T-Rex, and Google-Re (where T-Rex is further scoped into 1-1, N-1, and N-M relation types as well). Our results are direct extensions of Table 2 in \textit{Language Models are Knowledge Bases}?~\cite{petroni2019lama}. Importantly, LAMA only attempts to predict words from a common vocabulary that are a single token in the model's vocabulary. As we use the 57k GPT-2 BPE subword tokenizer, our results are directly comparable to GPT-2, but not to BERT which uses a different tokenizer. 

For the zero-shot question answering tasks, we use the official released evaluation splits of Trivia QA~\cite{joshi2017triviaqa}, Natural Questions~\cite{kwiatkowski2019natural}, and Web Questions~\cite{berant2013semantic} and evaluate with both exact match (EM) using the string generated after the last blank \texttt{Answer:} and before the next newline character, as well as whether any of the gold answers are contained as a substring in the generated string (in-EM), since language models are known to try to answer in complete sentences (\minh{example}). We normalize both gold and predicted answers. We filter Natural Questions to those with short answers as in the T5 paper~\cite{roberts2020much}: we ignore questions whose answers are longer than 5 tokens. We use the unfiltered version of the Trivia QA dataset. For both Natural Questions and Trivia QA datasets, we report the performance on the validation sets because the test sets with labels are not publicly available. 


For Edge Prob tasks, we train a separate classifier for each task~\footnote{We use the code provided at \url{https://github.com/
jsalt18-sentence-repl/jiant.}}. The input to the classifier is the top-layer hidden state obtained from the transformer-based encoder. Following~\cite{roberts2020much}, we freeze the encoder weights to prevent it from altering the internal representations toward specific tasks. We report $F_1$ performance based on the test set of each task. Furthermore, to analyze the encoder's behavior in the pretraining process, we also track its performance in the early stage of pretraining. Specifically, for every 1 thousand pretraining steps, we store the encoder checkpoint and repeat the Edge Prob benchmarking with this checkpoint.
% \cx{Minh can you write a couple sentences of how we use Edge Probe here?}

\textbf{Compared Methods.}
% \cx{state that we mainly compare with autoregressive GPT-2 style LM \tnlg{}, and we include comparisons with different sizes. and then the \kalm{} settings. Say that we also include some other method for reference but not for comparison.
% }
We mainly compare with the autoregressive GPT-2 architecture, versions of which we trained in house -- TNLG-12L, TNLG-24L, TNLG-1.5B, and TNLG-17B -- using the Megatron-LM codebase, the latter two requiring model parallelism of degree 2 and 4, respectively. We pretrain \kalm{} models that exactly mimic the architectures and training regimens of TNLG-12L and TNLG-24L.

% \cx{
% list and refer to the table of their parameters (embedding and transformer), inference time, state that the transformer parameters size is more indicate of model effectiveness, as in OpenAI paper~\cite{kaplan2020scaling} and also of inference efficiency.
% }

% \input{table/parameters}

In Table \ref{tab:parameters}} we describe the architectures of the models studied in this paper. The total number of parameters is more indicative of model quality, while the transformer layer parameters is more indicative of runtime~\cite{kaplan2020scaling}.



\textbf{Implementation Details.} 
% \cx{Describe some general details: training time on hardware, the input dropout, optimizer, etc. one paragraph only. If need to discuss more details, refer to appendix.}
We typically trained our models on either 32 or 64 Nvidia v100 GPUs in DGX-2 pods for 3-6 days. In all cases, we used the same linear learning rate warm-up over 3.2k steps to a maximum of 1.5e-4 using batch 512 sequences of length 1024, with cosine learning rate decay to a minimum of 1e-5 over at most 300k steps. Models were trained until convergence around 200-250k steps (no more than 4-5 epochs). Dropout of 0.1 was applied on the input tokens as well as in the attention layers; the model had $\ell$-2 regularization of 0.01. We always initialized all embedding matrices with a uniform normal. 

For \kalm{} we added an additional dropout on the linked entities, replacing them with the \texttt{null} entity 10\% of the time. We also sampled negatives for the output entity prediction task according to the following regimen: 1\% of the time the negative was the \texttt{null} entity, 49\% it was a random entity chosen from among all 1.4M, and the remaining 50\% it was a ``difficult'' negative chosen from among the closest 100 nearest Trans-E neighbors of the positive entity. We did not initialize the entity embeddings with Trans-E.   









==> arxiv/intro_outline.tex <==
\section{Introduction}


\cx{Our main contributions. 
\begin{enumerate}
    \item A simple and effective way to inject the knowledge awareness into NLG model pretraining, that brings the knowledge capacity out of transformer without changing its architecture.
    \item Strong performance in perplexity, word accuracy, LAMA test, and also real downstream application
    \item Analyses that shows what inductive bias our knowledge aware input and output injected to transformer, and how that influenced the pretraining process
\end{enumerate}
}


\cx{Outline:}

\cx{The promising advances of NLG and its usage in various applicaitons, especially with pretrained model.However, the concern of degeneration dull and not meaningful language, and even worth, semantically wrong language that will not be useful (PAA) or harm users.
}

\cx{Many attempts in trying to make language generation more grounded, trying leverage external knowledge as memory, intermediate layer, or copy from.}

\cx{Recent findings in BERT style representation model shows that transformer actually can capture many semantics. linguistic pipeline, lama, Aristo QA, and bigger models even start to capture semantic knowledge in traditional knowledge graphs. Yet there is a gap of 1) LAMA performance of NLG verus NLR models; 2) overlook study of how much knowledge the NLG (auto-regressive) style transformer can capture. Though there might be a higher standard impact of NLG systems: classification error or imprecet top 3 ranking is much better than providing a missleading or false information in NLG responses.}

\cx{Before relying on external knowledge bank as an add-on, this paper studies how much knowledge the vannila transformer architecture is able to capture, and how to unleash such inner semantic capabilities in language model pretraining.
We provide a simple knowledge-aware pretraining strategy: let the model know which token(s) are entities when taking input (Awareness) and also let the model know that we would like it to learn more semantic nuances in pretraining (Guidance). 
}


\cx{The awareness is done simply by adding another tokenizer, that tokenizes spans to entity ids using a simple dictionary look up. No disambiguation is added and we just let the model know the most popular potential entity id of the span.}

\cx{The guidance is simply add an entity prediction task that requires fine-grained semantic ability to distinguish similar entities from ANN.}


\cx{Both techniques communicate with the transformer, without changing any architecture or adding external storage. Yet it is proven to be very effective: better LAMA versus much much bigger models.
The KAG also makes the general LM better: better perplexity and better token level accuracy.}

\cx{The improved transformer can serve as drop-in replacement of GPT-2 and the gains in LM and Lama are generalizable to downstream NLG tasks.}

\cx{Provide insights on what is picked in the KAG training during the pretraining process. Also compare the behaviors of a smaller, but KAG pretrained, with once of the biggest NLG model (17B) parameters, show the differences of KAG and over-parameterization.}


==> arxiv/intro_v1.tex <==
\section{Introduction}


\cx{Our main contributions. 
\begin{enumerate}
    \item A simple and effective way to pack more knowledge into language model via knowledge-aware pretraining, without changing its architecture.
    \item Strong performance in perplexity, word accuracy, LAMA test, and also zero-shot QA, showing the improved knowledge capability, as a promising step towards unsupervised multi-task learning.
    \item Analyses that shows what inductive bias our knowledge aware input and output injected to transformer, how that influenced the pretraining process, and how that compared with the largest language model ever, 17 billion NLG.
\end{enumerate}
}


% \cx{Outline:}

% \cx{The promising advances of NLG and its usage in various applicaitons, especially with pretrained model.However, the concern of degeneration dull and not meaningful language, and even worth, semantically wrong language that will not be useful (PAA) or harm users.}

%language model pretraining
%the NLU versus NLG (autoregressive) and the importance of factual correctness in NLG results


Current pretrained language models can be viewed as either learning language representations via recovering the corrupted text sequence, e.g., Masked language modeling (MLM)~\cite{devlin2019bert}, Permutation language modeling~\cite{yang2019xlnet}, or Replaced Token Detection~\cite{clark2020electra}, via auto-regressive language modeling~\cite{radford2019language}, or combinations of the two~\cite{dong2019unified, raffel2019exploring}. MLM-style language models are often used in natural language representation/understanding (NLU) tasks, for example, achieving ``beyond human performance'' in GLUE tasks~\cite{wang2018glue} and question answering tasks~\cite{rajpurkar2016squad}. The auto-regressive language models are more often used in natural language generation (NLG), for example, providing ``human-like open-domain chatbot''~\cite{zhang2019dialogpt, adiwardana2020towards, roller2020recipes}.


The effectiveness of NLU language models has also been observed in real-world AI systems. 
In web search, BERT helps search engines better understand natural language queries and provided unparalleled improvements of search accuracies in major search engines~\cite{GoogleBert, BingBert}. 
In conversational AI, BERT effectively learns user's search trajectories and provides informative and useful conversational question suggestions, that are favored by actual search engine users~\cite{rosset2020leading}. 

Deploying auto-regressive NLG language models in real systems, on the other hand, raises more concerns than their NLU siblings. De-generating none-informative or factually incorrect language has long been a challenge of NLG models~\cite{li2019don, rosset2020leading, holtzman2019curious}. While a user might be lenient to some noises in the search results, but showing user an incorrectly generated contents such as ``Barack's wife is Hillary''~\cite{logan2019barack} likely leads to bad or even adversarial user experience.  


% \cx{Recent findings in BERT style representation model shows that transformer actually can capture many semantics. linguistic pipeline, lama, Aristo QA, and bigger models even start to capture semantic knowledge in traditional knowledge graphs. Yet there is a gap of 1) LAMA performance of NLG verus NLR models; 2) overlook study of how much knowledge the NLG (auto-regressive) style transformer can capture. Though there might be a higher standard impact of NLG systems: classification error or imprecet top 3 ranking is much better than providing a misleading or false information in NLG responses.}




% \cx{Before relying on external knowledge bank as an add-on, this paper studies how much knowledge the vannila transformer architecture is able to capture, and how to unleash such inner semantic capabilities in language model pretraining.
% We provide a simple knowledge-aware pretraining strategy: let the model know which token(s) are entities when taking input (Awareness) and also let the model know that we would like it to learn more semantic nuances in pretraining (Guidance). 
% }




% \cx{The awareness is done simply by adding another tokenizer, that tokenizes spans to entity ids using a simple dictionary look up. No disambiguation is added and we just let the model know the most popular potential entity id of the span.}

% \cx{The guidance is simply add an entity prediction task that requires fine-grained semantic ability to distinguish similar entities from ANN.}

In this paper we aim to improve the semantic and knowledge capability of auto-regressive transformer language models. Following the recent observations on the potential knowledge capability of transformer network~\cite{clark2020transformers, petroni2019lama, roberts2020much}, we refrain from adding external storage or intermediate entity layers~\cite{logan2019barack, hayashi2019latent, peters2019knowledge, fevry2020entities}, and seek to bring out the intrinsic knowledge ability from the vanilla transformer architecture, by making the network ``aware'' of semantics during pretraining.
Specifically, when pretraining, besides feeding in the token sequences to the transformer, we also conduct a fussy entity linking and feed the linked entity sequences as a \textit{knowledge-aware input} to the model; Similarly, besides asking to model to output the next token in the auto-regressive pretraining, we also require the model to provide \textit{knowledge-aware output} which is the next linked entity.




% \cx{The improved transformer can serve as drop-in replacement of GPT-2 and the gains in LM and Lama are generalizable to downstream NLG tasks.}

In practice, adding the knowledge-awareness input is as simple as using another entity-tokenizer that performs a dictionary look up and maps the n-grams (surface forms) to its most popular entity id (frequency based linking~\cite{inproceedings}); adding the knowledge-awareness output is to include a next entity prediction task in the pretraining tasks, using the same entity dictionary look up.
Both can be easily incorporated into the transformer language model with its vanilla architectures untouched.

% \cx{Both techniques communicate with the transformer, without changing any architecture or adding external storage. Yet it is proven to be very effective: better LAMA versus much much bigger models.
% The KAG also makes the general LM better: better perplexity and better token level accuracy.}

In our experiment, we instantiate the knowledge-aware pretraining on GPT-2, the auto-regressive transformer language model, and pretrain the model the same way as GPT-2, using the same transformer architecture, and the same network layers.
The knowledge-aware GPT-2, or KA-GPT2, show strong semantic capability in variation evaluations: in  all LAMA knowledge prob tasks~\cite{petroni2019lama}, KA-GPT2 outperforms GPT-2  that uses the same transformer network with more commonsense knowledge, factual knowledge, and better SQuAD test accuracy.
% all of which come from simply letting the network aware of entity semantics in pretraining. 
The advantage of knowledge awareness also helps transformers model the language better; we have observed much better language modeling perplexities and token-level accuracy in various transformer sizes. Simply letting the model aware of entity semantics in pretraining improves the parameter efficiency significantly---a 24 layer KA-GPT2 model with 345M transformer parameters can even matches the performance of a transformer langauge model that uses the same architecture but 17 billions parameters.
% All of these advantages come from simply letting the model aware of entity semantics in pretraining, without changing any network architecture

\cx{needs results from Minh to rewrite here.}
To better understand the advantage of knowledge-aware pretraining, we leverage the edge prob technique~\cite{tenney2019bert, tenney2019you} and dissect the \textit{learned language representations through the pretraining process}. Our results illustrate that the auto-regressive transformers start to learn the basis of language in the beginning of the pretraining, and gradually learns more complex semantics in the process, while adding knowledge-awareness greatly speed up the capture of more higher level semantics, e.g., coreferences and entity types, and also helps the model perform better in those more complicated tasks.
We also prob the representations learned in the 17 billion language model, compare the observations on the much smaller KA-GPT2 language model, and provide more insights of the differences and similarities between bruct-force over-parameterization and knowledge-awareness.


% \cx{Provide insights on what is picked in the KAG training during the pretraining process. Also compare the behaviors of a smaller, but KAG pretrained, with once of the biggest NLG model (17B) parameters, show the differences of KAG and over-parameterization.}








% \cx{Many attempts in trying to make language generation more grounded, trying leverage external knowledge as memory, intermediate layer, or copy from.}
% A common approach to improve the factual-correctness is to ground the language models on prior knowledge, i.e., maintaining the knowledge base/graph as an external memory~\cite{radford2019language, hayashi2019latent} or inject the entity information as additional representations through the transformer layers~\cite{peters2019knowledge, fevry2020entities}. 
% With access with such grounded knowledge, the generative model could avoid making artificial facts by directly copying from the external storage.



==> arxiv/method.tex <==
\section{Pretraining Knowledge-Aware Language Models}
In this section we first present preliminaries in language modeling and GPT-2 style auto-regressive models and then how we add knowledge-awareness in their pretraining.


\input{Preliminaries}


\subsection{Knowledge-Aware Pretraining}
As shown in Eqn.~\ref{eq.lm}, the pretraining is solely at the word level: it takes the previous word tokens in the text sequence, $w_{<i}$, and learns to predict the next word token $w_i$. All the semantics previously observed in the pretrained language models are captured by the transformer indirectly: the neural network may just find it beneficial for next word prediction to implicitly incorporate the entity typing semantics; there is no \textit{explicit} requirement to incorporate semantic knowledge.
Yet we expect the pretrained language models, for example, to generate factually correct statements when used in conversational agent, which perhaps were mainly achieved by lucky draws in their word distribution.

In this work we eliminate this discrepancy by making transformer networks aware of the need of knowledge in language model pretraining. Before stacking more layers or adding external knowledge storage for grounded language model, we use this knowledge-aware language modeling (\kalm{}) framework to pack more semantic knowledge into the same amount of transformer network parameters. As the first step of \kalm{}, the knowledge-awareness is simply achieved by an \textit{entity tokenizer} that forms an additional entity token sequence, in duet of the word token sequence~\cite{xiong2017duet}, to construct the \textit{knowledge-aware} language model pretraining.


\textbf{Entity Tokenizer} segments the text sequences into entity ids using a surface form dictionary, which maps the word n-grams (surface forms) into entity ids.
It simply uses maps each word n-grams to its most popular entity id:
$w_{i:i+k} \xrightarrow{\text{dict look up}}  e_i$, where $e_i$ is the most popular entity referred by the word k-gram $w_{i:i+k}$, and $e_i = \text{null}$ if the uni-gram is not part of a feasible surface name. 

This simple dictionary look-up operation can be conducted efficiently, similar to the (sub)word tokenizer, and the two forms the word-entity duet token sequence for the text:
\begin{align}
    X_\text{duet} &= \begin{cases}
    \{w_1,...,w_i,...,w_n\} & \text{Word Sequence;}\\
    \{e_1,...,e_i,...,e_n\} & \text{Entity Sequence.}
    \end{cases}
\end{align}
The two sequences are aligned position by position.
If a word is not part of an entity name, its corresponding position is filled with the ``null'' entity id. If multiple words together form an entity name, the corresponding entity id is duplicated to each position corresponding to these words.
For example, the name ``United States'' at $w_{i:i+2}$ is mapped to entity ``USA'' in $e_i$ and $e_{i+1}$.

Compared to previous work that uses a more precise entity linker to disambiguate or to use labeled entity annotations to learn this disambiguation~\cite{peters2019knowledge, fevry2020entities}, our minimalist choice of using a straightforward frequency-based dictionary look up emphasizes our goal of letting language models aware of the need to capture more knowledge themselves, instead of feeding them fine-grained knowledge information directly. 
The noise in this frequency-based mapping may also help regularize the pretraining as a corrupt input.

\subsection{Knowledge-Aware Language Models} 

The entity tokenizer is used in our knowledge-aware language modeling to inject the inductive bias towards entity semantics in the pretraining process. Formally, we define the conditional language model probability with the word-entity duet token sequence as the follows:
\begin{align}
    p_\text{duet} &= \prod_{i}p(w_i, e_i | w_{<i}, e_{<i})  \label{eq.klm}\\
    &= \prod_{i}p(w_i| w_{<i}, e_{<i}) p(e_i| w_{<i}, e_{<i}),
\end{align}
where we add the independence assumption between the probability of a token and its corresponding entity.

This formulate is parameterized in \kalm{} in two parts, the knowledge-aware input which models the conditioning on $w_{<i}, e_{<i}$, and the knowledge-aware output that learns the conditioned probabilities. Both uses standard auto-regressive transformer networks as in GPT-2~\cite{radford2019language}.

\textbf{Knowledge-Aware Input.} We use an entity embedding layer in the input to the transformer language model and combine it with the word embeddings:
\begin{align}
    \vec{e_i} &= \text{Embedding}_e(e_i),  \\
    \vec{w_i} &= \text{Embedding}_t(t_i).
\end{align}
The two embeddings are combined to form the knowledge-ware input:
\begin{align}
    \vec{t_i} &= \vec{w_i} + \vec{e_i}.
\end{align}
All the embeddings are learned in the language model pretraining. During training, we also have a \texttt{null} entity that is added to all non-entity-linked tokens, and we replace a percentage of entity-linked tokens with this \texttt{null} token to regularize the model. 

\textbf{Knowledge-Aware Output.} The knowledge-aware input is fed into standard transformer layers, the same as the word-only input. We use one output head for the word probability,  one for the entity, and share all transformer layers between words and entities. If there are $L$ transformers layers and $h_i^L$ is the output of the $i$'th token, the loss for position $i$ is computed as
% \cx{Corby: check the detailed formulation is the same with your implementation}:
\begin{align}
    h_i^L                 &= \texttt{transformer}^L(t_{<i}), \label{eqn.hidden}\\
    p(w_i|t_{<i})         &= \softmax(\texttt{Linear}_w(h_i^L)), \label{eqn.word}\\
    \text{s}(h_i^L, e_j)    &= \texttt{cos}(\texttt{Linear}_e(h_i^L), e_j)    \label{eqn.score}\\
    \ell_e(e_i|t_{<i}, e_n) &= \texttt{max}(0, \text{s}(h_i^L, e_i) - \text{s}(h_i^L, e_n) + \lambda). \label{eqn.entity}
\end{align}
The transformer layer in Eqn.~\ref{eqn.hidden} can be stacked multiple times similar with in GPT-2. The scoring function in Eqn.~\ref{eqn.score} simply projects the hidden state into the embedding space with $\texttt{Linear}_e$ and takes the cosine similarity with entity vector $e_j$. Assuming that position $i$ is linked by our entity linker to $e_i$, we choose a corresponding negative entity $e_n$ to contrast with $e_i$ using margin loss with margin $\lambda$ in Eqn.~\ref{eqn.entity}. 

\textbf{Pretraining.} The knowledge-aware input and output are incorporated in the standard multi-task set up for our \kalm{} knowledge-aware language model pretraining:
\begin{align}
 l_\text{\kalm}(X_\text{duet}) &= \prod_{i}l_w(p(w_i|t_{<i})) + \alpha \ell_e(e_i|t_{<i}, e_n). \label{eqn.loss}
\end{align}
It combines the word modeling loss $l_w()$ with the entity modeling loss $l_e()$, with $\alpha$ the hyper-parameter to balance the importance of the two.
The word loss $l_w()$ is the same as standard auto-regressive language modeling. The entity loss is slightly different as the entity vocabulary is bigger than the sub-word vocabulary, thus we use the margin loss:
\begin{align}
    l_e(p(e_i|t_{<i})) &= \text{relu}[1-(p(e_i|t_{<i}) - p(e_i^-|t_{<i}))],
\end{align}
that contrast the positive entity $e_i$ with the sampled negative entity $e_i^-$.

\textbf{Inference.} The inference of the pretrained \kalm{}, e.g., in generation tasks, can simply use the word prediction head $p(w_i|t_{<i})$, which is consistent with the word only language models, e.g., GPT-2. 

In this way the entity prediction task is an auxiliary task that guides the model to attend to the entity semantics during pretraining; in inference only the shared transformer representations is used. Compared with the standard GPT-2 style language models, 
the architecture of \kalm{} only differs with an enlarged tokenization vocabulary with additional entity tokens, and their entity embeddings before the input to the transformer network.
The transformer architecture and its layers configurations are kept consistent; only the network parameters are learned with knowledge-aware pretraining.





==> arxiv/overall.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{clll|lllllll}
                       &                            & Wiki-103 & Lambada   & \multicolumn{1}{l|}{G-Re}  & \multicolumn{4}{c|}{T-REx}                               & \multicolumn{1}{l|}{C-Net} & Squad \\ \cline{3-11} 
\multicolumn{2}{c}{Model}                           & Perplex. & last word & \multicolumn{1}{l|}{Total} & 1-1     & N-1     & N-M     & \multicolumn{1}{l|}{Total} & \multicolumn{1}{l|}{Total} & Total \\ \hline
\multirow{2}{*}{Bert}  & \multicolumn{1}{l|}{base}  & -        & -         & 9.9                        & 68.0    & 32.4    & 24.7    & 31.1                       & 15.6                       & 14.1  \\
                       & \multicolumn{1}{l|}{large} & -        & -         & 10.5                       & 74.5    & 34.2    & 24.3    & 32.3                       & 19.2                       & 17.4  \\ \hline
\multirow{2}{*}{GPT-2} & \multicolumn{1}{l|}{-24L}  & 26.37    & ???       &                            & 56.03   & 19.76   & 19.93   &                            &                            &       \\
                       & \multicolumn{1}{l|}{-1.5B} & 17.48    & 52.66     &                            & 62.31   & 21.53   & 19.61   &                            &                            &       \\ \hline
\multirow{4}{*}{TNLG}  & \multicolumn{1}{l|}{-12L}  & 20.85    & 33.73     & 215k                       & 19.94+  & 12.65+  & 14.5+   &                            &                            &       \\
                       & \multicolumn{1}{l|}{-24L}  & 21.40+    & 42.63+     & 100k                       & 36.18+  & 17.56+  & 17.41+  &                            &                            &       \\
                       & \multicolumn{1}{l|}{-1.5B} & 14.68+   & 56.72+    & 100k                       & 65.04+  & 24.04+  & 21.51+  &                            &                            &       \\
                       & \multicolumn{1}{l|}{-17B}  & 10.21    & 67.98     & 300k                       & 76.82   & 29.60   & 27.14   & 30.95                      &                            &       \\ \hline
\multirow{2}{*}{KALM}  & \multicolumn{1}{l|}{-12L}  & 22.51    & 40.26     & 100k                       & 43.72+  & 23.74+  & 23.04+  & 24.44+                     &                            &       \\
                       & \multicolumn{1}{l|}{-24L}  &          &           & 80k                        & 66.37++ & 22.52++ & 23.28++ & 24.96++                    &                            &      
\end{tabular}
    \caption{\cx{The Wikitext language model results and LAMA knowledge prob results of generation models. Follow the table format of LAMA paper Table 2, add perplexity and lamada as two extra rows on top. Include GPT-2 baselines and our models (final version + ablation of input awareness and output awareness individually). Also include the BERT-base and BERT-large baseline results on the same LAMA subsets (if they are directly comparable this way).}}
    \label{tab:lmoverall}
\end{table}

%\begin{tabular}{llllllllllllll}
% \multicolumn{1}{c}{Corpus} & \multicolumn{1}{c}{Relation} & \multicolumn{2}{c}{Statistics} & \multicolumn{2}{c|}{Bert Baselines} & \multicolumn{2}{c|}{GPT-2} & \multicolumn{4}{c|}{TNLG}   & \multicolumn{2}{c|}{KALM} \\ \hline
%                           &                              & \#            & \# Rel         & base             & large            & -24L         & -1.5B       & -12L & -24L & -1.5B & -17B  & -12L        & -24L        \\
% Wiki-103                   & Perplex.                     & ???           & -              & -                & -                & 26.37        & 17.48       &      &      &       & 10.21 &             &             \\ \hline
% Lambada                    & last word                    & ???           & -              & -                & -                & ???          & 52.66       &      &      &       & 67.98 &             &             \\ \hline
% \multirow{4}{*}{Google-Re} & birth-pl.                    & 2.9k          & 1              & 14.9             & 16.1             &              &             &      &      &       &       &             &             \\
%                           & birth-date                   & 1.8k          & 1              & 1.5              & 1.4              &              &             &      &      &       &       &             &             \\
%                           & death-pl.                    & 700           & 1              & 13.1             & 14.0             &              &             &      &      &       &       &             &             \\ \cline{2-14} 
%                           & total                        & 5.5k          & 3              & 9.9              & 10.5             &              &             &      &      &       &       &             &             \\ \hline
% \multirow{4}{*}{T-REx}     & 1-1                          & 900           & 2              & 68.0             & 74.5             &              &             &      &      &       &       &             &             \\
%                           & N-1                          & 20k           & 23             & 32.4             & 34.2             &              &             &      &      &       &       &             &             \\
%                           & N-M                          & 13k           & 16             & 24.7             & 24.3             &              &             &      &      &       &       &             &             \\ \cline{2-14} 
%                           & Total                        & 34k           & 41             & 31.1             & 32.3             &              &             &      &      &       &       &             &             \\ \hline
% Conc. Net                  & Total                        & 11k           & 16             & 15.6             & 19.2             &              &             &      &      &       &       &             &             \\ \hline
% Squad                      & Total                        & 300           & -              & 14.1             & 17.4             &              &             &      &      &       &       &             &             \\ \hline
% \end{tabular}


==> table/ablation.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{c|c}
         &  \\
         & 
    \end{tabular}
    \caption{\cx{Ablation results on language model tasks, Lama (aggregated metrics), and perhaps on one evaluations. Ablation variations of our model: KALM with input only, KALM with output only, KALM with input only but all surface forms linked to one same entity id, KALM with output only but instead of prediciton entity from ANN, prediction entity from random entity neighbor; KALM (output) but just add more language model loss of surface names' tokens, instead of the entity prediction tasks---this is the salience span mask task in REALLm and T5-QA paper.}}
    \label{tab:ablation}
\end{table}

==> table/casestudy.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{c|c}
         &  \\
         & 
    \end{tabular}
    \caption{\cx{examples that show the factual correctness of our NLG results in LAMA, pick examples from several categories. This can be in appendix}}
    \label{tab:case}
\end{table}

==> table/dataSizes.tex <==
\begin{table}
    \centering
    \begin{tabular}{llll}
    Dataset           & Subset                            & \# Items & \# Rels \\ \hline
    Wikitext-103      & \multicolumn{1}{l|}{test split}   &          & -       \\
    Lambada           & \multicolumn{1}{l|}{}             &          & -       \\ \hline
    LAMA Google-Re    & \multicolumn{1}{l|}{}             & 4.6k     & 3       \\
    LAMA T-Rex        & \multicolumn{1}{l|}{1-1}          & 937      & 2       \\
    LAMA T-Rex        & \multicolumn{1}{l|}{N-1}          & 20k      & 23      \\
    LAMA T-Rex        & \multicolumn{1}{l|}{N-M}          & 13k      & 16      \\
    LAMA ConceptNet   & \multicolumn{1}{l|}{}             & 11k      & 16      \\
    LAMA Squad        & \multicolumn{1}{l|}{}             & 305      & -       \\ \hline
    Trivia QA         & \multicolumn{1}{l|}{}             & 11k      & -       \\
    Natural Questions & \multicolumn{1}{l|}{short-answer???} & 3.7k     & -       \\
    \end{tabular}
\end{table}

==> table/parameters.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{lllllll}
    Name                            & Trans. Params & Total Params & Layers & Hidden Dim & Attn Heads & runtime \\ \hline
    \multicolumn{1}{l|}{GPT-2}      & 355M               & 355M         & 24     & 1024       & 16         & ?       \\
    \multicolumn{1}{l|}{GPT-2 1.5B} & 1542M              & 1.5B         & 48     & 1600       & 16         & ?       \\ \hline
    \multicolumn{1}{l|}{TNLG-12L}   & 128M?              & 128M         & 12     & 768        & 12         & ?       \\
    \multicolumn{1}{l|}{TNLG-24L}   & 355M               & 355M         & 24     & 1024       & 16         & ?       \\
    \multicolumn{1}{l|}{TNLG-1.5B}  & 1542               & 1542M        & 48     & 1600       & 16         & ?       \\
    \multicolumn{1}{l|}{TNLG-17B}   & 17000M?            & 17000M       & 78     & 4256       & 28         & ?       \\ \hline
    \multicolumn{1}{l|}{KALM-12L}   & 128M?              & 553M         & 12     & 768        & 12         & ?       \\
    \multicolumn{1}{l|}{KALM-24L}   & 355M               & 780M         & 24     & 1024       & 16         & ?      
    \end{tabular}
\end{table}
